CoSLight: Co-optimizing Collaborator Selection and Decision-making to Enhance Traffic Signal Control

Effective multi-intersection collaboration is pivotal for reinforcement-learning-based traffic signal control to alleviate congestion. Existing work mainly chooses neighboring intersections as collaborators. However, quite an amount of congestion, even some wide-range congestion, is caused by non-neighbors failing to collaborate. To address these issues, we propose to separate the collaborator selection as a second policy to be learned, concurrently being updated with the original signal-controlling policy. Specifically, the selection policy in real-time adaptively selects the best teammates according to phase- and intersection-level features. Empirical results on both synthetic and real-world datasets provide robust validation for the superiority of our approach, offering significant improvements over existing state-of-the-art methods. The code is available at https://github.com/bonaldli/CoSLight.

==> 1-intro-new.tex <==
\section{Introduction}
% cooperation: (1) 和谁合作；（2）合作 + 决策 co-learn
% p1: intro of tsc
% (1)
% p2: 现有的marl是定义和谁合作，以及他们的问题
% p3: selling point: learning-based; based on their representation (dynamic/adaptive)
% (2)
% p4: 现有的 合作 | 决策 独立：他们的问题： 决策的upper bound取决于上一步的合作边界--> suboptimal
% p5: selling point: jointly optimize

% \mhy{According to the template, table Caption should be under the table body.}

Traffic Signal Control (TSC) plays a critical role in managing urban traffic flow and alleviating congestion. Over the past decade, multi-agent reinforcement learning (MARL) has emerged as a powerful tool for optimizing TSC~\citep{wei2019survey}. 
However, effectively promoting multi-intersection collaboration remains a persistent challenge in applying MARL to TSC.

Current MARL methods addressing multi-intersection collaboration, termed as Multi-intersection RL (MIRL), \revise{primarily focus on enhancing decision-making through representation extraction \re{and information aggregation} between intersections.}
Prominent works include those based on graph neural networks (GNNs)~\citep{wei2019colight,wu2021dynstgat,lou2022meta,devailly2021ig,yu2021macar}, as well as approaches utilizing multi-level embeddings~\citep{liang2022oam,oroojlooy2020attendlight,zhang2021attentionlight}. 
\revise{These methods tend to assume geographically adjacent intersections as natural collaborators. However, relying solely on topological proximity for selecting collaborators may not always yield optimal results~\citep{wu2021inductive,zhong2023contrastive}.}
\revise{
For instance, during \re{morning} rush hours, signals from residential to business areas must strategically coordinate to facilitate driving in town. As shown in Figure~\ref{fig:intro}(a), intersections in upper streams should regulate incoming traffic to prevent downstream congestion, requiring them to synchronize with signals closer to business districts, which direct traffic towards parking and alternate routes. This coordination goes beyond mere proximity, emphasizing the need for dynamic and non-adjacent collaboration across the network. \re{Likewise, during evening rush hours in Figure~\ref{fig:intro}(b), signals from business to residential areas also need to cooperate for better driving out of town. The two cooperations in the morning and evening peaks mostly differ due to different origin-destination flows and other factors such as weather and trip purpose.}
% For instance, in a grid-like road network, the signal at the top-left corner controls entry flows, while the signal at the bottom-right corner manages exit flows. During peak congestion, the top-left signal must limit entries, while the bottom-right maximizes exits. Despite not being directly connected, their coordination is vital for efficient traffic management across the network. This scenario illustrates that basing collaborator selection merely on topological structures can overlook essential dynamic and non-adjacent collaboration.
}
Thus, this poses the first challenge: How can we \textbf{dynamically} \textbf{select} the most suitable collaborators?

% todo1: 图示 
% todo2: 
    % 挑战1 与 例子 的引入
    % 市区：：： case  外围路口 早高峰 控制外围入口信号灯；出城xxx；晚高峰 出口与入口；更real～
% method 推导
% GAT backbone 的结果

% wu2021inductive,zhong2023contrastive: 动态邻接矩阵比KNN等方法好
% \ziyue{add citation}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/intro_pre-4.pdf}
	\caption{{(a)-(b): The coordination between signals during rush hours; (c)-(d): The collaboration policy $\boldsymbol{\rho}$ and decision policy $\boldsymbol{\theta}$ should be jointly optimized to prevent suboptimal.}
 % \ziyue{the fontsize of $\rho$ and $\theta$ inside (c)-(d) should be larger}} 
 }
    \label{fig:intro}
    \vspace{-10pt}
\end{figure}



\revise{
Moreover, the collaborator selection's quality profoundly decides the decision policy's upper bound. 
The prevalent practice is to \re{select collaborators without training first, and then to decide the signal policy}, as shown in Figure~\ref{fig:intro}(c). As a result, decision policy is optimized separately and may easily reach a suboptimal result \re{when the collaboration selection is bad}. Figure~\ref{fig:intro}(d) indicates that the joint optimization of the two policies can mutually steer each other towards better outcomes, thereby achieving the optimums simultaneously. This presents the second challenge: How can we establish a \textbf{strong coupling} between collaborator selection and decision policy to \textbf{jointly optimize} the overall goal of maximizing cumulative reward?
}



\revise{
Recognizing these limitations, we propose a novel strategy for multi-intersection collaboration in TSC. Our approach, which we term top-$k$ \textbf{Co}llaborator \textbf{S}election (CoS) policy, is combined with a dual-feature extractor, addressing the following challenges:\vspace{5pt} \\ 
}
\textbf{Challenge 1: Whom to cooperate with for the best?}
\begin{itemize}
    \item {\nameOurs~effectively extracts both phase-level based on FRAP \citep{zheng2019learning} and intersection-level representations based on Transformer~\citep{vaswani2017attention}: The dual features are used to \textit{adaptively} search the most beneficial intersections to collaborate.} 
    \item \revise{ \re{Being in real-time, the collaborator selection must be light and agile.} Unlike existing methods relying on heavy GNNs, we utilize a more \re{cost-efficient} two-layer MLP structure for top-$k$ collaborator selection. This design not only reduces computational complexity~\citep{han2022mlpinit, mlpmixer2021, wang2023gfs} but also surprisingly achieves better performance.}
    \item {Moreover, we incorporate two golden rules in the MLP collaboration matrix: that ``\textit{you are your biggest collaborator}'' and ``\textit{mutual reciprocity}'', which penalize the diagonal to be the largest and the matrix to be symmetric. \re{These rules significantly improve collaboration benefits.}}
\end{itemize}
\textbf{Challenge 2: Jointly optimize collaboration policy and decision policy?} 
We design a joint optimization scheme that simultaneously trains the~\abbr~and decision policy to maximize the cumulative return \revise{through joint policy gradient}, reinforcing the strong coupling between collaboration policy and decision policy. 

By addressing these challenges, our approach improves the performance of TSC, not only at individual intersections but also across the entire traffic network. 
%\revise{Comprehensive experiments conducted on both synthetic and real datasets demonstrate the effectiveness of our approach, showing better improvements compared to existing methods.}




==> 1-intro-old.tex <==
\section{Introduction}
% cooperation: (1) 和谁合作；（2）合作 + 决策 co-learn
% p1: intro of tsc
% (1)
% p2: 现有的marl是定义和谁合作，以及他们的问题
% p3: selling point: learning-based; based on their representation (dynamic/adaptive)
% (2)
% p4: 现有的 合作 | 决策 独立：他们的问题： 决策的upper bound取决于上一步的合作边界--> suboptimal
% p5: selling point: jointly optimize

% \mhy{According to the template, table Caption should be under the table body.}

Traffic Signal Control (TSC) plays a critical role in managing urban traffic flow and alleviating congestion. Over the past decade, multi-agent reinforcement learning (MARL) has emerged as a powerful tool for optimizing TSC~\citep{wei2019survey}. 
However, effectively promoting multi-intersection collaboration remains a persistent challenge in applying MARL to TSC.

Current MARL methods addressing multi-intersection collaboration, termed as Multi-intersection RL (MIRL), \revise{primarily focus on enhancing decision-making through representation extraction between intersections.}
% focus on enhancing the intersection decision-making by introducing collaborator representations based on cross-intersection representation extraction. 
Prominent works include those based on graph neural networks (GNNs)~\citep{wei2019colight,wu2021dynstgat,lou2022meta,devailly2021ig,yu2021macar}, as well as approaches utilizing multi-level embeddings~\citep{liang2022oam,oroojlooy2020attendlight,zhang2021attentionlight}. 
\revise{These methods tend to assume geographically adjacent intersections as natural collaborators. However, relying solely on topological proximity for selecting collaborators may not always yield optimal results~\citep{wu2021inductive,zhong2023contrastive}.}
% {However, these methods either assume all other intersections as collaborators and refine to only the geographical neighbors as collaborators, which may introduce irrelevant interferences that can disrupt decision-making~\citep{wu2021inductive,zhong2023contrastive}.} 
\revise{
For instance, in a grid-like road network, the signal at the top-left corner controls entry flows, while the signal at the bottom-right corner manages exit flows. 
% consider the interplay between two traffic signals: one at the top-left corner controlling vehicle entry, and another at the bottom-right managing exit flows. 
During peak congestion, the top-left signal must limit entries, while the bottom-right maximizes exits. 
Despite not being directly connected, their coordination is vital for efficient traffic management across the network.
This scenario illustrates that basing collaborator selection merely on topological structures can overlook essential dynamic and non-adjacent collaboration.
}
This poses the first challenge: How can we \textbf{dynamically} \textbf{select} the most suitable collaborators?
% This poses 
% wu2021inductive,zhong2023contrastive: 动态邻接矩阵比KNN等方法好
% \ziyue{add citation}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.99\linewidth]{fig/intro_pre-2.pdf}
	\caption{{(a)-(b): The careful choice when selecting collaborator: In some cases, it is hop-1 neighbors, and considering hop-3 neighbors brings no gain compared to without cooperation. In other cases, it could be different; (c)-(d): The collaboration policy $\boldsymbol{\rho}$ and decision policy $\boldsymbol{\theta}$ should be jointly optimized to prevent suboptimal.} 
 }
    \label{fig:intro}
    \vspace{-10pt}
\end{figure}

Figure~\ref{fig:intro}(a) showcases our preliminary experimental results, wherein an intersection is nominated as the center, and collaborators are heuristically chosen within 1, 2, and 3-hop distances, respectively. Figure~\ref{fig:intro}(b) demonstrates the reward gains compared to without cooperation as the distance increases. {It shows that the hop-1 neighbors are the best to cooperate with. However, in another scenario (in Appendix~\ref{app:hops}), 2-hop is the best. Moreover, when considering even more factors, such as road structure or traffic similarity, it is even harder to decide whom to collaborate with.} The quality of the collaborator selection profoundly decides the upper bound of decision policy. Therefore, it is crucial to adaptively select the most suitable collaborators.
% The results suggest the significant influence of the choice of collaborative teammates on the outcomes. Thus, the challenge lies in the dynamic selection of the most appropriate collaborators.

% Furthermore, the quality of the collaborator selection profoundly decides the upper bound of decision policy. 
The prevalent practice of selecting collaborators without training, as shown in Figure~\ref{fig:intro}(c), entails that the decision policy is optimized separately and may easily reach a suboptimal result. Figure~\ref{fig:intro}(d) indicates that the iterative optimization of the two policies can mutually steer each other towards more optimal outcomes, thereby achieving the optimal outcomes simultaneously. This presents the second challenge: How can we establish a \textbf{strong coupling} between collaborator selection and decision policy to \textbf{jointly optimize} the overall goal of maximizing cumulative reward?

% Furthermore, the quality of the collaborative selection profoundly influences the upper bound of decision policy optimization.
% Figure~\ref{fig:intro}(c) 
% The prevalent practice of manually selecting a fixed number of collaborators decouples the integral relationship between collaborator selection and decision policy, potentially leading to suboptimal outcomes.
% This presents the second challenge: How can we establish a \textbf{strong coupling} between \textbf{collaborator selection} and \textbf{decision policy} to jointly optimize the overall goal of maximizing cumulative reward?

% Furthermore, the upper bound of decision policy optimization directly depends on the quality of teammate selection. Manually selecting a fixed number of teammates for heuristic collaboration decouples the inherent  relationship between teammate selection and decision policy, leading to suboptimal solutions. Hence, a mechanism should be developed to foster a strong coupling between multi-intersection collaboration selection and decision policy, aiming at joint optimization of the ultimate goal of maximizing cumulative reward.

% The existing RL methods for handling multi-intersection collaboration, referred to as Multi-intersection RL (or MIRL for short), can be divided into three categories.
% The first category employs a single agent as a central controller to develop passage plans for all intersections~\citep{lee2019reinforcement,kim2019cooperative}. These methods suffer from the curse of dimensionality, as the decision space grows exponentially with an increasing number of intersections. 
% The second category controls each intersection by an independent agent that can retrieve global information during training~\citep{mannion2016experimental,prashanth2011reinforcement,chen2020toward,su2022emvlight}.  This form of collaboration is implicit, as the information required for cooperating intersections can only propagate via gradients~\citep{yu2022surprising}, leading to weak collaboration. 
% The third category comprises methods that augment the decision-making of single intersections by introducing representations of neighboring intersections based on cross-intersection representation extraction, \hl{such as graph neural network-based methods}~\citep{wei2019colight,wu2021dynstgat,lou2022meta,devailly2021ig,yu2021macar}, and multi-level embeddings~\citep{liang2022oam,oroojlooy2020attendlight,zhang2021attentionlight}. \hl{Nonetheless, these methods, which use either neighboring intersections or select neighbors based on distance or even use all intersections as neighbors, have the risk of introducing irrelevant interferences, thereby disrupting precise decision-making.} Furthermore, these methods decouple the crucial link between multi-intersection collaboration and intersection decision-making through their representation extraction and multi-intersection selection scheme.
% These issues consequently pose three pivotal research questions:
% RQ1: How to derive \textbf{powerful representation} for multi-intersections?
% RQ2: How to \textbf{adaptively identify the optimal intersections} for collaboration?
% RQ3: How to establish a \textbf{strong coupling} between multi-intersection collaboration selection and decision policy to jointly optimize the ultimate goal for the cumulative environmental reward?


To address the challenges outlined above, we propose an innovative strategy for multi-intersection collaboration in TSC. Our approach introduces {a well-designed and easy-to-implement} coordination policy named top-$k$ \textbf{Co}llaborator \textbf{S}election (\abbr) policy combined with a dual-feature extractor. 
For the two challenges of collaboration, our approach tackles them in the following ways: \vspace{5pt} \\ 
% \vspace{15pt}
\textbf{Challenge 1: Whom to cooperate with for the optimal reward?}
\begin{itemize}
    \item {\nameOurs~effectively extracts both phase-level based on FRAP \cite{zheng2019learning} and intersection-level representations based on Transformer~\cite{vaswani2017attention}: The dual feature will be used to \textit{adaptively} search the most beneficial intersections to collaborate.} %and reinforces the coupling between multi-intersection collaboration and decision policy. %With a dual-feature extractor, we derive robust and informative representations for multi-intersections. These representations effectively capture both phase-specific and intersection-specific features, leading to a more accurate understanding of intersection dynamics.
    %\item Our~\abbr~effectively discerns the representations of the most appropriate intersections for collaboration, thus reducing the risk of incorporating irrelevant interferences.
    % Our TCS adaptively identifies the optimal intersections for collaboration. 
    % This selection process is based on the feature representations of intersections, \mhy{why?} which minimizes the risk of incorporating irrelevant interferences.
    % \item {As mentioned before, quite some existing methods rely on GNN-based methods (e.g., GATs) to select collaborators. However, besides the risk of introducing noise, another disadvantage is: GNNs are commonly implemented by sparse matrix multiplication, which is very slow even on GPUs. This hinders the application to large-scale cities. A new trend is happening now in the general spatiotemporal domain, that MLPs could already be enough \cite{han2022mlpinit, mlpmixer2021, wang2023gfs}. Thus, we also stacked two-layer MLP to decide the top-$k$ collaborators, which also surprisingly demonstrates the strongest performance.}
    \item Many existing methods utilize GNNs, like Graph Attention Networks (GATs), for collaborator selection. Yet, these can introduce noise and are very slow even on GPUs due to sparse matrix multiplication, limiting their use in large-scale cities. Recent trends in the spatiotemporal domain suggest that MLPs might suffice and converge faster \cite{han2022mlpinit, mlpmixer2021, wang2023gfs}. Accordingly, we employed two-layer MLPs for top-$k$ collaborator selection, achieving superior performance.
    \item {Moreover, we incorporate two rules in the MLP collaboration matrix: that ``\textit{you are your biggest collaborator}'' and ``\textit{mutual reciprocity}'', which penalize the diagonal to be the largest and the matrix to be symmetric.}
\end{itemize}
\textbf{Challenge 2: Jointly optimize collaboration policy and decision policy?} 
% {Following in a similar manner as EM-algorithm~\cite{ng2012algorithm},} 
We design a joint optimization regime that simultaneously trains the~\abbr~and decision policy to maximize the cumulative return, reinforcing the strong coupling between collaboration policy and decision policy. 

By addressing these challenges, our approach significantly improves the performance of TSC, not only at individual intersections but also across the entire traffic network. Comprehensive experiments conducted on both synthetic and real datasets validate the superiority of our approach over existing methods.





==> 1-intro.tex <==
\section{Introduction}
% cooperation: (1) 和谁合作；（2）合作 + 决策 co-learn
% p1: intro of tsc
% (1)
% p2: 现有的marl是定义和谁合作，以及他们的问题
% p3: selling point: learning-based; based on their representation (dynamic/adaptive)
% (2)
% p4: 现有的 合作 | 决策 独立：他们的问题： 决策的upper bound取决于上一步的合作边界--> suboptimal
% p5: selling point: jointly optimize

% \mhy{According to the template, table Caption should be under the table body.}

Traffic Signal Control (TSC) plays a critical role in managing urban traffic flow and alleviating congestion. Over the past decade, multi-agent reinforcement learning (MARL) has emerged as a powerful tool for optimizing TSC~\citep{wei2019survey}. 
However, effectively promoting multi-intersection collaboration remains a persistent challenge in applying MARL to TSC.

Current MARL methods addressing multi-intersection collaboration, termed as Multi-intersection RL (MIRL), \revise{primarily focus on enhancing decision-making through representation extraction between intersections.}
% focus on enhancing the intersection decision-making by introducing collaborator representations based on cross-intersection representation extraction. ruan2022gcs,hao2023gat,jiang2018graph,bohmer2020deep
Prominent works include those based on graph neural networks (GNNs)~\citep{wei2019colight,wu2021dynstgat,lou2022meta,devailly2021ig,yu2021macar,ruan2022gcs,bohmer2020deep}, as well as approaches utilizing multi-level embeddings~\citep{liang2022oam,oroojlooy2020attendlight,zhang2021attentionlight,hao2023gat,jiang2018graph,ruan2024made}. 
\revise{These methods tend to assume geographically adjacent intersections as natural collaborators. However, relying solely on topological proximity for selecting collaborators may not always yield optimal results~\citep{wu2021inductive,zhong2023contrastive}.}
% {However, these methods either assume all other intersections as collaborators and refine to only the geographical neighbors as collaborators, which may introduce irrelevant interferences that can disrupt decision-making~\citep{wu2021inductive,zhong2023contrastive}.} 
\revise{
For instance, in a grid-like road network, the signal at the top-left corner controls entry flows, while the signal at the bottom-right corner manages exit flows. 
% consider the interplay between two traffic signals: one at the top-left corner controlling vehicle entry, and another at the bottom-right managing exit flows. 
During peak congestion, the top-left signal must limit entries, while the bottom-right maximizes exits. 
Despite not being directly connected, their coordination is vital for efficient traffic management across the network.
This scenario illustrates that basing collaborator selection merely on topological structures can overlook essential dynamic and non-adjacent collaboration.
}
This poses the first challenge: How can we \textbf{dynamically} \textbf{select} the most suitable collaborators?

% todo1: 图示 
% todo2: 
    % 挑战1 与 例子 的引入
    % 市区：：： case  外围路口 早高峰 控制外围入口信号灯；出城xxx；晚高峰 出口与入口；更real～
% method 推导
% GAT backbone 的结果





% This poses 
% wu2021inductive,zhong2023contrastive: 动态邻接矩阵比KNN等方法好
% \ziyue{add citation}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.99\linewidth]{fig/intro_pre-3.pdf}
	\caption{{The collaboration policy $\boldsymbol{\rho}$ and decision policy $\boldsymbol{\theta}$ should be jointly optimized to prevent suboptimal.} 
 }
    \label{fig:intro}
    \vspace{-10pt}
\end{figure}


\revise{
Moreover, the quality of the collaborator selection profoundly decides the upper bound of decision policy. 
The prevalent practice of selecting collaborators without training, as shown in Figure~\ref{fig:intro}(a), entails that the decision policy is optimized separately and may easily reach a suboptimal result. Figure~\ref{fig:intro}(b) indicates that the joint optimization of the two policies can mutually steer each other towards more optimal outcomes, thereby achieving the optimal outcomes simultaneously. This presents the second challenge: How can we establish a \textbf{strong coupling} between collaborator selection and decision policy to \textbf{jointly optimize} the overall goal of maximizing cumulative reward?
}



\revise{
Recognizing these limitations, we propose a novel strategy for multi-intersection collaboration in TSC. Our approach, which we term top-$k$ \textbf{Co}llaborator \textbf{S}election (CoS) policy, is combined with a dual-feature extractor, addressing the following challenges:\vspace{5pt} \\ 
}
% To address the challenges outlined above, we propose an innovative strategy for multi-intersection collaboration in TSC. Our approach introduces a top-$k$ \textbf{Co}llaborator \textbf{S}election (\abbr) policy combined with a dual-feature extractor. 
% For the two challenges of collaboration, our approach tackles them in the following ways: \vspace{5pt} \\ 
% \vspace{15pt}
\textbf{Challenge 1: Whom to cooperate with for the optimal reward?}
\begin{itemize}
    \item {\nameOurs~effectively extracts both phase-level based on FRAP \citep{zheng2019learning} and intersection-level representations based on Transformer~\citep{vaswani2017attention}: The dual feature will be used to \textit{adaptively} search the most beneficial intersections to collaborate.} 
    \item \revise{ Unlike existing methods that rely on GNNs, our approach utilizes a more efficient two-layer MLP structure for top-$k$ collaborator selection. This design not only reduces computational complexity~\citep{han2022mlpinit, mlpmixer2021, wang2023gfs} but also achieves better performance.}
    % Many existing methods utilize GNNs, like Graph Attention Networks (GATs), for collaborator selection. Yet, these can introduce noise and are very slow even on GPUs due to sparse matrix multiplication, limiting their use in large-scale cities. Recent trends in the spatiotemporal domain suggest that MLPs might suffice and converge faster \citep{han2022mlpinit, mlpmixer2021, wang2023gfs}. Accordingly, we employed two-layer MLPs for top-$k$ collaborator selection, achieving superior performance.
    \item {Moreover, we incorporate two rules in the MLP collaboration matrix: that ``\textit{you are your biggest collaborator}'' and ``\textit{mutual reciprocity}'', which penalize the diagonal to be the largest and the matrix to be symmetric.}
\end{itemize}
\textbf{Challenge 2: Jointly optimize collaboration policy and decision policy?} 
% {Following in a similar manner as EM-algorithm~\citep{ng2012algorithm},} 
We design a joint optimization regime that simultaneously trains the~\abbr~and decision policy to maximize the cumulative return \revise{through joint policy gradient}, reinforcing the strong coupling between collaboration policy and decision policy. 

By addressing these challenges, our approach improves the performance of TSC, not only at individual intersections but also across the entire traffic network. 
\revise{Comprehensive experiments conducted on both synthetic and real datasets demonstrate the effectiveness of our approach, showing better improvements compared to existing methods.}
% Comprehensive experiments conducted on both synthetic and real datasets validate the superiority of our approach over existing methods.


% Therefore, it is crucial 
% Figure~\ref{fig:intro}(a) showcases our preliminary experimental results, wherein an intersection is nominated as the center, and collaborators are heuristically chosen within 1, 2, and 3-hop distances, respectively. Figure~\ref{fig:intro}(b) demonstrates the reward gains compared to without cooperation as the distance increases. {It shows that the hop-1 neighbors are the best to cooperate with. However, in another scenario (in Appendix~\ref{app:hops}), 2-hop is the best. Moreover, when considering even more factors, such as road structure or traffic similarity, it is even harder to decide whom to collaborate with.} The quality of the collaborator selection profoundly decides the upper bound of decision policy. Therefore, it is crucial to adaptively select the most suitable collaborators.

% The results suggest the significant influence of the choice of collaborative teammates on the outcomes. Thus, the challenge lies in the dynamic selection of the most appropriate collaborators.

% Furthermore, the quality of the collaborator selection profoundly decides the upper bound of decision policy. 
% The prevalent practice of selecting collaborators without training, as shown in Figure~\ref{fig:intro}(c), entails that the decision policy is optimized separately and may easily reach a suboptimal result. Figure~\ref{fig:intro}(d) indicates that the iterative optimization of the two policies can mutually steer each other towards more optimal outcomes, thereby achieving the optimal outcomes simultaneously. This presents the second challenge: How can we establish a \textbf{strong coupling} between collaborator selection and decision policy to \textbf{jointly optimize} the overall goal of maximizing cumulative reward?

% Furthermore, the quality of the collaborative selection profoundly influences the upper bound of decision policy optimization.
% Figure~\ref{fig:intro}(c) 
% The prevalent practice of manually selecting a fixed number of collaborators decouples the integral relationship between collaborator selection and decision policy, potentially leading to suboptimal outcomes.
% This presents the second challenge: How can we establish a \textbf{strong coupling} between \textbf{collaborator selection} and \textbf{decision policy} to jointly optimize the overall goal of maximizing cumulative reward?

% Furthermore, the upper bound of decision policy optimization directly depends on the quality of teammate selection. Manually selecting a fixed number of teammates for heuristic collaboration decouples the inherent  relationship between teammate selection and decision policy, leading to suboptimal solutions. Hence, a mechanism should be developed to foster a strong coupling between multi-intersection collaboration selection and decision policy, aiming at joint optimization of the ultimate goal of maximizing cumulative reward.

% The existing RL methods for handling multi-intersection collaboration, referred to as Multi-intersection RL (or MIRL for short), can be divided into three categories.
% The first category employs a single agent as a central controller to develop passage plans for all intersections~\citep{lee2019reinforcement,kim2019cooperative}. These methods suffer from the curse of dimensionality, as the decision space grows exponentially with an increasing number of intersections. 
% The second category controls each intersection by an independent agent that can retrieve global information during training~\citep{mannion2016experimental,prashanth2011reinforcement,chen2020toward,su2022emvlight}.  This form of collaboration is implicit, as the information required for cooperating intersections can only propagate via gradients~\citep{yu2022surprising}, leading to weak collaboration. 
% The third category comprises methods that augment the decision-making of single intersections by introducing representations of neighboring intersections based on cross-intersection representation extraction, \hl{such as graph neural network-based methods}~\citep{wei2019colight,wu2021dynstgat,lou2022meta,devailly2021ig,yu2021macar}, and multi-level embeddings~\citep{liang2022oam,oroojlooy2020attendlight,zhang2021attentionlight}. \hl{Nonetheless, these methods, which use either neighboring intersections or select neighbors based on distance or even use all intersections as neighbors, have the risk of introducing irrelevant interferences, thereby disrupting precise decision-making.} Furthermore, these methods decouple the crucial link between multi-intersection collaboration and intersection decision-making through their representation extraction and multi-intersection selection scheme.
% These issues consequently pose three pivotal research questions:
% RQ1: How to derive \textbf{powerful representation} for multi-intersections?
% RQ2: How to \textbf{adaptively identify the optimal intersections} for collaboration?
% RQ3: How to establish a \textbf{strong coupling} between multi-intersection collaboration selection and decision policy to jointly optimize the ultimate goal for the cumulative environmental reward?



==> 2-pre.tex <==
\section{Preliminary}


% movement
% phase
% intersection

In this section, we lay the groundwork by introducing some fundamental concepts related to traffic signal control. These concepts provide a necessary foundation for understanding our proposed multi-intersection collaboration strategy for TSC. The notions we will cover include traffic movement, signal phase, traffic intersection, multi-intersection traffic signal control, queue length, and pressure.
In Figure~\ref{fig:pre}, we give a visual representation of these concepts to further aid understanding.

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/pre.pdf}
	\caption{The illustration of the proposed framework.}
    \label{fig:pre}
\end{figure*}



\subsection{Traffic Intersection}
A traffic intersection is where two or more roads cross each other. Traffic signals at intersections control the flow of traffic, ensuring vehicles from different directions can safely navigate the intersection. Traffic intersections are often hotspots for congestion, making their efficient management crucial for overall traffic flow.
In the left part of Figure~\ref{fig:pre}, there is a 4-arm intersection. It contains some lanes, such as left lane, through lane, and right lane.
Specifically, there are four incoming (outgoing) roads and twelve incoming (outgoing) lanes.
The incoming lane is for entering vehicles, and the outgoing lane is for exiting vehicles.
Here, we denote the set of incoming lanes and the set of outgoing lanes in the intersection $i$ as $\mathcal{L}^i_{in}$, and $\mathcal{L}^i_{out}$, respectively.


\subsection{Traffic Movement}
Traffic movement refers to the progression of vehicles across an intersection in a specific direction, namely, turning left, going straight, or turning right. 
As depicted in Figure~\ref{fig:pre}, twelve distinct traffic movements can be identified. Note that in this paper, right-turning vehicles may proceed irrespective of the signal status.


\subsection{Signal Phase}
A traffic signal phase represents a set of allowable traffic movements at an intersection. Within a phase, specific traffic directions are coordinated to flow smoothly without conflicting with others. As illustrated in Figure~\ref{fig:pre}, the intersection comprises eight distinct phases, with phase $F$ currently activated.



\subsection{Multi-Intersection Traffic Signal Control (TSC)}
At each intersection, an RL agent is deployed to manage the traffic signal control. During each time unit denoted as $t_{duration}$,  the RL agent $i$ observes the state of the environment, represented as $o^i_t$. It then determines the action $a^i_t$, which dictates the signal phase for intersection $i$. The objective of the agent $i$ is to choose an optimal action (i.e., determining the most appropriate signal phase ) to maximize the cumulative reward.

\subsection{Queue Length}
The queue length at each intersection $i$ is defined as the aggregate length of vehicle queues in all incoming lanes toward the intersection, denoted as:
\begin{equation}
    Q^i_{len} = \sum{q(l)}, l \in \mathcal{L}^i_{in},
\end{equation}
where $q(l)$ is the queue length in the lane $l$.

\subsection{Pressure}
Pressure, a crucial concept in traffic signal control, can be categorized into two types: intersection-wise pressure and phase-wise pressure.
\begin{itemize}
    \item Intersection-wise pressure represents the difference between the aggregate of queued vehicles on all incoming lanes and the total queued vehicles on all outgoing lanes at a specific intersection. This measurement helps to understand the traffic load imbalance within the intersection.
    \item Phase-wise pressure, on the other hand, relates to specific signal phases. Each signal phase, denoted as $p$, permits several traffic movements, each marked by $(l, m)$. If $x(l, m)$ signifies the difference in the number of vehicles between lane $l$ and lane $m$ for a given traffic movement $(l, m)$, then the pressure of a signal phase, $P(p)$, is essentially the cumulative sum of the pressures of all permissible movements within that phase, i.e., $\sum _{(l,m)} x(l, m)$, for all $(l, m)$ that belong to the phase $p$.
\end{itemize}




Understanding these basic concepts is critical for discussing and comprehending the techniques used in traffic signal control and the specifics of our proposed method.



==> 3-1-dual-feature-old.tex <==

\subsubsection{Dual-Feature Extractor.}
% \ziyue{I think too much attention is put on the feature extraction. It can be easily summarized as two paragraphs: FRAP for phase, and attention for intersection.}
To ensure accurate and effective policy-making in TSC, obtaining a comprehensive representation of traffic situations is essential. 
%To achieve this, we introduce a dual-feature extractor module that captures features from both the phase and intersection levels, providing a holistic view of the road network.
{While extracting features at the phase level provides useful information for individual intersections, it is insufficient to achieve optimal coordination across multiple intersections, as traffic flows at correlated intersections also exert influence. Therefore, in addition to phase-level representations, we also extract features at the intersection level to capture the network-level traffic dynamics required for effective multi-intersection signal control.}

At the \textbf{phase} level, we adopt FRAP~\citepp{zheng2019learning} to obtain the phase-wise representation. 
The raw observations $o$ from the simulator include $K$ features, such as the number of vehicles, queue length, the current phase, the flow, etc. For any traffic movement $m, m \in \{1,...,8\}$ in an intersection $i$, the $k$-th feature in the raw observation can be denoted as $o_{m,k}^i$. For brevity, the superscript $i$ is omitted hereinafter.
First, the embedding of traffic movement $m$ is obtained by Multi-Layer Perceptron (MLP):
\begin{equation} 
\bm{e}_{m} = ||_{k=1}^K Sigmoid(MLP_k(o_{m,k})),
\end{equation} 
where $||$ denotes concatenation, and $Sigmoid$ is the activation function.
Then FRAP module is applied to extract the phase competition representation, denoted as follows.
\begin{equation}
    \bm{e}_{pcr} = FRAP(\bm{e}_{m_1},...,\bm{e}_{m_8}).
\end{equation}
The process can be summarized as follows.
(a) Phase embedding: Each phase $p$ consists of two movements $m_1, m_2$, and we get the phase embedding $\bm{e}_p = \bm{e}_{m_1} + \bm{e}_{m_2}$.
(b) Phase pair representation: For any pair $p_k, p_l$ from different phases, the pairwise relation vector is $\bm{e}_{p_k, p_l} = \bm{e}_{p_k} || \bm{e}_{p_l}$. Gathering the vectors of all phase pairs can obtain the pair demand embedding volume $\bm{E}$. Then the phase pair representation can be denoted as $\bm{e}_{ppr} = Conv_{1 \times 1}(\bm{E})$, where $Conv_{1 \times 1}$ is the convolutional layer with 1 × 1 filters. 
(c) Phase competition: Let $\bm{M}$ be phase competition mask, and the phase competition representation can be obtained by: $\bm{e}_{pcr} = Conv_{1 \times 1}(\bm{e}_{ppr} \otimes \bm{M})$, where $\otimes$ is the element-wise multiplication. Here, we reshape $\bm{e}_{pcr}$ as a vector through \textit{flatten} operation.

Finally, an MLP is utilized to mine the phase representation in the intersection $i$ as follows.
\begin{equation}
    \bm{e}^i_{pr} = MLP(\bm{e}_{pcr})
\end{equation}


At the \textbf{intersection} level, we adopt the Transformer encoder~\citep{vaswani2017attention} as the backbone to model the relationship across multiple intersections.
The Transformer encoder takes in the phase representations $\bm{e}_{pr} = \{\bm{e}^i_{pr}\}_{i=1}^N, \bm{e}_{pr} \in \mathbb{R}^{N \times d}$, where $N$ is the number of intersections, $d$ is the input dimension.
Given three learnable matrices $W_q \in \mathbb{R}^{d \times d_k}, W_k \in \mathbb{R}^{d \times d_k}, W_v \in \mathbb{R}^{d \times d_v}$, 
the multi-head scaled dot product attention can be calculated as follows, enabling the model to jointly attend to information from different representation subspaces..
\begin{equation}
    Q^{(h)}, K^{(h)}, V^{(h)} = \bm{e}_{pr}W_q^{(h)}, \bm{e}_{pr}W_k^{(h)}, \bm{e}_{pr}W_v^{(h)},
\end{equation}
% \begin{equation}
%     head^{(h)} = Attention(Q^{(h)}, K^{(h)}, V^{(h)})= softmax\left ( \frac{Q^{(h)}{K^{(h)}}^{\rm{T}} }{\sqrt{d_k} }  \right ) V^{(h)},
% \end{equation}
\begin{equation}
    head^{(h)} =  softmax\left ( \frac{Q^{(h)}{K^{(h)}}^{\rm{T}} }{\sqrt{d_k} }  \right ) V^{(h)},
\end{equation}
\begin{equation}
    \bm{e}_M = MultiHead(\bm{e}_{pr})=||_{h=1}^{H} head^{(h)} 
\cdot  W_O,
\end{equation}
where $d_k, d_v$ are the hyper-parameters, $H$ is the number of attention heads, 
the superscript $h$ represents the head index,
and $W_O \in \mathbb{R}^{h \cdot d_v \times d}$ is the learnable matrix. 

% the scaled dot product attention can be calculated as follows.
% \begin{equation}
%     Q, K, V = \bm{e}_{pr}W_q, \bm{e}_{pr}W_k, \bm{e}_{pr}W_v,
% \end{equation}
% \begin{equation}
%     Attention(Q, K, V) = softmax\left ( \frac{QK^{T} }{\sqrt{d_k} }  \right ) V,
% \end{equation}
% where $d_k, d_v$ is the hyper-parameter.

% To obtain rich representation, multi-head attention is applied, enabling the model to jointly attend to information from different representation subspaces.
% The calculation can be formulated as follows.
% \begin{equation}
%     Q^{(h)}, K^{(h)}, V^{(h)} = \bm{e}_{pr}W_q^{(h)}, \bm{e}_{pr}W_k^{(h)}, \bm{e}_{pr}W_v^{(h)},
% \end{equation}
% \begin{equation}
%     head^{(h)} = Attention(Q^{(h)}, K^{(h)}, V^{(h)}),
% \end{equation}
% \begin{equation}
%     \bm{e}_M = MultiHead(\bm{e}_{pr})=||_{h=1}^{H} head^{(h)} 
% \cdot  W_O,
% \end{equation}
% where $H$ is the number of attention heads, 
% the superscript $h$ represents the head index,
% and $W_O \in \mathbb{R}^{h \cdot d_v \times d}$ is the learnable matrix. 

Then a point-wise feed-forward network (FFN) is applied.
\begin{equation}
   FFN(\bm{e}_M) = max(0, \bm{e}_M W_1+b_1)W_2+b_2,
    % \bm{e}_M' = LayerNorm(\bm{e}_{pr} + Dropout(\bm{e}_M)),
\end{equation}
where $W_1 \in \mathbb{R}^{d \times d_f}, W_2 \in \mathbb{R}^{d_f \times d}, b_1 \in \mathbb{R}^{d_f}, b_2 \in \mathbb{R}^{d}$ are learnable parameters, $d_f$ is the hyper-parameter.

So far, the intersection-wise representation is obtained.
\begin{equation}
    \bm{e}_{ir} = FFN(\bm{e}_M), \ \ \bm{e}_{ir} \in \mathbb{R}^{N \times d}.
\end{equation}
% where $$.

In summary, by extracting features from both the phase level and intersection level simultaneously, we are able to obtain a more comprehensive insight to provide sufficient representation for subsequent modeling.









